UniForm: A Reuse Attention Mechanism Optimized for Efficient Vision Transformers on Edge Devices

Transformer-based architectures have demonstrated remarkable success across various domains, but their deployment on edge devices remains challenging due to high memory and computational demands. In this paper, we introduce a novel Reuse Attention mechanism, tailored for efficient memory access and computational optimization, enabling seamless operation on resource-constrained platforms without compromising performance. Unlike traditional multi-head attention (MHA), which redundantly computes separate attention matrices for each head, Reuse Attention consolidates these computations into a shared attention matrix, significantly reducing memory overhead and computational complexity. Comprehensive experiments on ImageNet-1K and downstream tasks show that the proposed UniForm models leveraging Reuse Attention achieve state-of-the-art imagenet classification accuracy while outperforming existing attention mechanisms, such as Linear Attention and Flash Attention, in inference speed and memory scalability. Notably, UniForm-l achieves a 76.7% Top-1 accuracy on ImageNet-1K with 21.8ms inference time on edge devices like the Jetson AGX Orin, representing up to a 5x speedup over competing benchmark methods. These results demonstrate the versatility of Reuse Attention across high-performance GPUs and edge platforms, paving the way for broader real-time applications

==> sec/5_relatedwork.tex <==
\section{Related Works}
\label{sec:related_works}

\textbf{Computational Complexity in Multi-Head Attention}:
Multi-head attention requires multiple matrix multiplications for each head, significantly increasing computational demands. Vaswani et al. (2017) introduced the Transformer architecture, which employs MHA to capture diverse aspects of the input data. Subsequent studies have highlighted the computational burden of these operations (Raganato \& Tiedemann, 2020).

\textbf{Single-Head vs. Multi-Head Attention}:
Studies comparing single-head and multi-head attention, such as Michel et al. (2019), suggest that the performance gap between them is not as substantial as previously assumed. This finding opens the door to optimizing MHA by reducing redundancy in computations.

\textbf{Importance of Values in Attention Mechanisms}:
The role of values in attention mechanisms, while crucial, has not received as much attention as queries and keys. Recent pruning studies indicate that values are less sensitive to pruning, suggesting their relative redundancy (Voita et al., 2019).

\textbf{MixConv and Kernel Diversity}:
MixConv (Tan \& Le, 2019) demonstrated that using diverse kernel sizes can enhance model performance by capturing varied spatial features. This concept can be extended to the value computation in attention mechanisms to introduce diversity and robustness.
